MDGAN: Boosting Anomaly Detection Using \\Multi-Discriminator Generative Adversarial Networks

Anomaly detection is often considered a challenging field of machine learning due to the difficulty of obtaining anomalous samples for training and the need to obtain a sufficient amount of training data. In recent years, autoencoders have been shown to be effective anomaly detectors that train only on "normal" data. Generative adversarial networks (GANs) have been used to generate additional training samples for classifiers, thus making them more accurate and robust. However, in anomaly detection GANs are only used to reconstruct existing samples rather than to generate additional ones. This stems both from the small amount and lack of diversity of anomalous data in most domains. In this study we propose MDGAN, a novel GAN architecture for improving anomaly detection through the generation of additional samples. Our approach uses two discriminators: a dense network for determining whether the generated samples are of sufficient quality (i.e., valid) and an autoencoder that serves as an anomaly detector. MDGAN enables us to reconcile two conflicting goals: 1) generate high-quality samples that can fool the first discriminator, and 2) generate samples that can eventually be effectively reconstructed by the second discriminator, thus improving its performance. Empirical evaluation on a diverse set of datasets demonstrates the merits of our approach.

==> Datasets.tex <==
%\subsection{Datasets}




%Datasets used for anomaly detection in our experiments are NSL-KDD, MNIST and  Kitsune data set video injection. Data sets were divided into a train and test sets. In order to train our models in a semi-supervised manner, only benign (normal) data was used for training. The test set contains both normal and anomalous data.
%\begin{itemize}
%\item NSL-KDD - a bench mark data set for the task of network intrusion detection systems (NIDS), containing only selected records from the original KDD cup 99 dataset. Since the KDDCup contains a huge amount of duplicate data records, it will make the learning algorithm biased. Thus NDL-KDD data set was created and is adopted for NIDS evaluation. The training contains 67343 non-malicious observations. The test set contains 9711 non-malicious observations and 12833 malicious observations.
%We preprocessed the data set as followed: 1) symbolic features were transformed into one-hot encoding -except 'flag' and 'service' that were dropped due to their large possibilities,(2) only the 'normal' records from the training set were used for the training process - this is done in order the use semi-supervised training of the autoencoder.


%\item MNIST \yotam{remove?} - data set that contains images of handwritten digits. We created 10 different training sets, each time dropping the anomalous digit from the training set. Evaluation was done on the entire MNIST test set, labeling the normal digits as 0 and the anomaly digit as 1. Images were flatten before insertion to the framework. 

%\item Video Injection (Kitsune ADD CITE) - data set that contains parsed pcaps of an attacker the injects a recorded video clip into a live video stream. In kitsune they've extracted features from each packetsm features such as packet's arrival time, size and network addresses.  The data set contains 2,472,401 packets, of which 102499 are malicious. We used the first 1 million observations for training, which does not contain anomalies. The test set contains the rest of the data.

%\item Pendigits - a multi-class classification dataset having 10 classes (0 - 9). The database is created by collecting 250 samples from 44 different writes. We used a transformme version of the original dataset (CITE  F. Keller, E. Muller, K. Bohm.“HiCS: High-contrast subspaces for density-based outlier ranking.” ICDE, 2012.   Saket Sathe and Charu C. Aggarwal. LODES: Local Density meets Spectral Outlier Detection. SIAM Conference on Data Mining, 2016.) The data set contains 6,870 instances, from which 534 are anomalies. Training was done using 6,000 normal instances.

%\item Annthyroid - a binary-class classification data set. The problem is to determine whether a patient referred to the clinic is hypothyroid or not. The data set contains 7,200 instances, from which 534 are anomalies. Training was done using 6,000 normal instances. (CITE Abe, Naoki, Bianca Zadrozny, and John Langford. “Outlier detection by active learning.” Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining. ACM, 2006.

%Liu, Fei Tony, Kai Ming Ting, and Zhi-Hua Zhou. “Isolation forest.” 2008 Eighth IEEE International Conference on Data Mining. IEEE, 2008.

%K. M. Ting, J. T. S. Chuan, and F. T. Liu. “Mass: A New Ranking Measure for Anomaly Detection.“, IEEE Transactions on Knowledge and Data Engineering, 2009.)


%\item Forest Cover - a multi-class classification data set that is used predicting forest cover type from cartographic variables only. We've used a transform version of the original data set (CITE http://odds.cs.stonybrook.edu/forestcovercovertype-dataset/). The data set contains 286,048 instances, from which 2,747 are anomalies. Training was done using 250,000 normal instances.

%\end{itemize}



%\pagebreak


==> autoencoder_alg.tex <==
% \section{Algorithm 1: Autoencoder}


\begin{algorithm}
\caption{Autoencoder training}\label{alg:ae}
\begin{algorithmic}[1]
\Procedure{fit}{$autoencoder,DATA, epochs$}



\State \textbf{return} $autoencoder$
\EndProcedure
\end{algorithmic}
\end{algorithm}
